Efficient Learning and Computation of Linear Correlated Equilibrium in General Convex Games

We propose efficient no-regret learning dynamics and ellipsoid-based methods for computing linear correlated equilibria$\unicode{x2014}$a relaxation of correlated equilibria and a strengthening of coarse correlated equilibria$\unicode{x2014}$in general convex games. These are games where the number of pure strategies is potentially exponential in the natural representation of the game, such as extensive-form games. Our work identifies linear correlated equilibria as the tightest known notion of equilibrium that is computable in polynomial time and is efficiently learnable for general convex games. Our results are enabled by a generalization of the seminal framework of of Gordon et al. [2008] for $\Phi$-regret minimization, providing extensions to this framework that can be used even when the set of deviations $\Phi$ is intractable to separate/optimize over. Our polynomial-time algorithms are similarly enabled by extending the Ellipsoid-Against-Hope approach of Papadimitriou and Roughgarden [2008] and its generalization to games of non-polynomial type proposed by Farina and Pipis [2024a]. We provide an extension to these approaches when we do not have access to the separation oracles required by these works for the dual player.

==> figs/algo_step1v2.tex <==


\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=0.5 ]   (192.9,202.7) -- (207.05,245.32) ;
\draw [shift={(208,248.17)}, rotate = 251.63] [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.5 ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- (4.74,0) -- cycle    ;
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=0.04 ][dash pattern={on 3pt off 3pt}][line width=0.75]  (34.79,226.25) .. controls (46.27,204.49) and (64.13,223.43) .. (79.65,215.01) .. controls (95.16,206.6) and (106.56,182.19) .. (123.21,198.55) .. controls (139.86,214.92) and (125.37,241.29) .. (138.4,251.8) .. controls (151.43,262.31) and (158.86,286.3) .. (135.4,298.2) .. controls (111.94,310.1) and (109.89,296.69) .. (98.72,294.85) .. controls (87.56,293) and (78.4,302.17) .. (71.4,304.6) .. controls (64.4,307.03) and (55.4,306.2) .. (46.2,298.6) .. controls (37,291) and (44.34,285.98) .. (41,269) .. controls (37.66,252.02) and (23.32,248) .. (34.79,226.25) -- cycle ;
\draw  [fill={rgb, 255:red, 255; green, 226; blue, 99 }  ,fill opacity=1 ][line width=0.75]  (80.28,261.54) .. controls (74.74,253.81) and (76.52,243.05) .. (84.25,237.51) .. controls (91.98,231.97) and (102.74,233.75) .. (108.28,241.48) .. controls (113.82,249.21) and (112.04,259.97) .. (104.31,265.51) .. controls (96.58,271.05) and (85.82,269.27) .. (80.28,261.54) -- cycle ;
\draw [line width=1.5]    (36.4,254.2) .. controls (28.4,272.2) and (35.4,294.2) .. (66.4,295.2) ;
\draw  [draw opacity=0] (237.12,253.55) .. controls (225.28,263.85) and (209.82,270.08) .. (192.9,270.08) .. controls (155.68,270.08) and (125.52,239.92) .. (125.52,202.7) .. controls (125.52,176.82) and (140.1,154.35) .. (161.5,143.06) -- (192.9,202.7) -- cycle ; \draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ] (237.12,253.55) .. controls (225.28,263.85) and (209.82,270.08) .. (192.9,270.08) .. controls (155.68,270.08) and (125.52,239.92) .. (125.52,202.7) .. controls (125.52,176.82) and (140.1,154.35) .. (161.5,143.06) ;  
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=0.5 ]   (192.9,202.7) -- (175.42,264.51) ;
\draw [shift={(174.6,267.4)}, rotate = 285.79] [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.5 ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- (4.74,0) -- cycle    ;
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.4 ][line width=1.5]  (125.75,209.25) .. controls (145.25,218.25) and (124.6,208.9) .. (145,218.6) .. controls (143.5,241) and (144.5,229.5) .. (143,247.25) .. controls (131.5,236.25) and (127,221.5) .. (125.75,209.25) -- cycle ;
\draw [line width=1.5]    (36.4,254.2) -- (75.4,184.2) -- (145,218.6) -- (139.4,301.2) -- (66.4,295.2) ;
\draw  [draw opacity=0][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (190.4,202.7) .. controls (190.4,201.32) and (191.52,200.2) .. (192.9,200.2) .. controls (194.28,200.2) and (195.4,201.32) .. (195.4,202.7) .. controls (195.4,204.08) and (194.28,205.2) .. (192.9,205.2) .. controls (191.52,205.2) and (190.4,204.08) .. (190.4,202.7) -- cycle ;
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][dash pattern={on 0.84pt off 2.51pt}] (144.97,202.7) .. controls (144.97,176.23) and (166.43,154.77) .. (192.9,154.77) .. controls (219.37,154.77) and (240.83,176.23) .. (240.83,202.7) .. controls (240.83,229.17) and (219.37,250.63) .. (192.9,250.63) .. controls (166.43,250.63) and (144.97,229.17) .. (144.97,202.7) -- cycle ;
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (137.25,229) -- (116.4,321.4) ;

\draw (183.8,181.4) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \phi $};
\draw (60.5,237) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \Phi $};
\draw (7.5,210) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \Phi _{\text{FP}}$};
\draw (53,175.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \tilde{\Phi }$};
\draw (179.2,246) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ] [align=left] {$\displaystyle \textcolor[rgb]{0.29,0.56,0.89}{q}$};
\draw (199.4,205.8) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ] [align=left] {$\displaystyle \textcolor[rgb]{0.29,0.56,0.89}{q-\delta }$};
\draw (93.2,319.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {$\displaystyle \mathcal{F:=B}( \phi ,q) \cap \tilde{\Phi }$};


==> figs/algo_step2av2.tex <==
\draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.4 ][line width=0.75]  (514.55,78.85) .. controls (534.05,87.85) and (513.4,78.5) .. (533.8,88.2) .. controls (532.3,110.6) and (533.3,99.1) .. (531.8,116.85) .. controls (520.3,105.85) and (515.8,91.1) .. (514.55,78.85) -- cycle ;
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=0.04 ][dash pattern={on 3pt off 3pt}][line width=0.75]  (423.59,96.1) .. controls (435.07,74.34) and (452.93,93.28) .. (468.45,84.86) .. controls (483.96,76.45) and (495.36,52.04) .. (512.01,68.4) .. controls (528.66,84.77) and (514.17,111.14) .. (527.2,121.65) .. controls (540.23,132.16) and (547.66,156.15) .. (524.2,168.05) .. controls (500.74,179.95) and (498.69,166.54) .. (487.52,164.7) .. controls (476.36,162.85) and (467.2,172.02) .. (460.2,174.45) .. controls (453.2,176.88) and (444.2,176.05) .. (435,168.45) .. controls (425.8,160.85) and (433.14,155.83) .. (429.8,138.85) .. controls (426.46,121.87) and (412.12,117.85) .. (423.59,96.1) -- cycle ;
\draw  [fill={rgb, 255:red, 255; green, 226; blue, 99 }  ,fill opacity=1 ][line width=0.75]  (469.08,131.14) .. controls (463.54,123.41) and (465.32,112.65) .. (473.05,107.11) .. controls (480.78,101.57) and (491.54,103.35) .. (497.08,111.08) .. controls (502.62,118.81) and (500.84,129.57) .. (493.11,135.11) .. controls (485.38,140.65) and (474.62,138.87) .. (469.08,131.14) -- cycle ;
\draw [line width=1.5]    (425.2,123.8) .. controls (417.2,141.8) and (424.2,163.8) .. (455.2,164.8) ;
\draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (516.45,92.05) .. controls (516.45,90.67) and (517.57,89.55) .. (518.95,89.55) .. controls (520.33,89.55) and (521.45,90.67) .. (521.45,92.05) .. controls (521.45,93.43) and (520.33,94.55) .. (518.95,94.55) .. controls (517.57,94.55) and (516.45,93.43) .. (516.45,92.05) -- cycle ;
\draw [line width=1.5]    (425.2,123.8) -- (464.2,53.8) -- (533.8,88.2) -- (528.2,170.8) -- (455.2,164.8) ;

\draw (449,103) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \Phi $};
\draw (406,71.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \Phi _{\text{FP}}$};
\draw (443.5,38.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \tilde{\Phi }$};
\draw (501.78,85.47) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {$\displaystyle \phi '$};
\draw (560.2,89.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {Terminate};


==> figs/algo_step2bv2.tex <==
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.4 ][line width=1.5]  (502.58,305.79) .. controls (508.63,308.5) and (504.38,306.5) .. (510.87,309.67) .. controls (513.88,317.5) and (518.38,327.25) .. (523.5,340.25) .. controls (525.38,350) and (526.63,358) .. (529,370.6) .. controls (503.63,345.5) and (502.63,321) .. (502.58,305.79) -- cycle ;
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=0.04 ][dash pattern={on 3pt off 3pt}][line width=0.75]  (429.99,331.85) .. controls (441.47,310.09) and (459.33,329.03) .. (474.85,320.61) .. controls (490.36,312.2) and (501.76,287.79) .. (518.41,304.15) .. controls (535.06,320.52) and (520.57,346.89) .. (533.6,357.4) .. controls (546.63,367.91) and (554.06,391.9) .. (530.6,403.8) .. controls (507.14,415.7) and (505.09,402.29) .. (493.92,400.45) .. controls (482.76,398.6) and (473.6,407.77) .. (466.6,410.2) .. controls (459.6,412.63) and (450.6,411.8) .. (441.4,404.2) .. controls (432.2,396.6) and (439.54,391.58) .. (436.2,374.6) .. controls (432.86,357.62) and (418.52,353.6) .. (429.99,331.85) -- cycle ;
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=0.3 ][dash pattern={on 0.84pt off 2.51pt}] (510.87,309.67) -- (523.5,340.25) -- (528.5,367.75) -- (534.6,406.8) -- (540.2,324.2) -- cycle ;
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=0.3 ][dash pattern={on 0.84pt off 2.51pt}] (481.43,295.14) -- (458.99,310.64) -- (470.6,289.8) -- cycle ;
\draw  [fill={rgb, 255:red, 255; green, 226; blue, 99 }  ,fill opacity=1 ][line width=0.75]  (475.48,367.14) .. controls (469.94,359.41) and (471.72,348.65) .. (479.45,343.11) .. controls (487.18,337.57) and (497.94,339.35) .. (503.48,347.08) .. controls (509.02,354.81) and (507.24,365.57) .. (499.51,371.11) .. controls (491.78,376.65) and (481.02,374.87) .. (475.48,367.14) -- cycle ;
\draw [line width=1.5]    (431.6,359.8) .. controls (423.6,377.8) and (430.6,399.8) .. (461.6,400.8) ;
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=0.5 ]   (588.1,308.3) -- (510.22,280.02) ;
\draw [shift={(507.4,279)}, rotate = 19.95] [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.5 ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- (4.74,0) -- cycle    ;
\draw  [draw opacity=0][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (585.6,308.3) .. controls (585.6,306.92) and (586.72,305.8) .. (588.1,305.8) .. controls (589.48,305.8) and (590.6,306.92) .. (590.6,308.3) .. controls (590.6,309.68) and (589.48,310.8) .. (588.1,310.8) .. controls (586.72,310.8) and (585.6,309.68) .. (585.6,308.3) -- cycle ;
\draw  [draw opacity=0][dash pattern={on 0.84pt off 2.51pt}] (632.32,359.15) .. controls (620.48,369.45) and (605.02,375.68) .. (588.1,375.68) .. controls (550.88,375.68) and (520.72,345.52) .. (520.72,308.3) .. controls (520.72,286.48) and (531.09,267.08) .. (547.17,254.77) -- (588.1,308.3) -- cycle ; \draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][dash pattern={on 0.84pt off 2.51pt}] (632.32,359.15) .. controls (620.48,369.45) and (605.02,375.68) .. (588.1,375.68) .. controls (550.88,375.68) and (520.72,345.52) .. (520.72,308.3) .. controls (520.72,286.48) and (531.09,267.08) .. (547.17,254.77) ;  
\draw  [draw opacity=0] (632.55,381.99) .. controls (619.58,389.84) and (604.37,394.35) .. (588.1,394.35) .. controls (540.58,394.35) and (502.05,355.82) .. (502.05,308.3) .. controls (502.05,285.12) and (511.22,264.07) .. (526.13,248.6) -- (588.1,308.3) -- cycle ; \draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ] (632.55,381.99) .. controls (619.58,389.84) and (604.37,394.35) .. (588.1,394.35) .. controls (540.58,394.35) and (502.05,355.82) .. (502.05,308.3) .. controls (502.05,285.12) and (511.22,264.07) .. (526.13,248.6) ;  
\draw [line width=1.5]    (431.6,359.8) -- (458.99,310.64) -- (481.43,295.14) -- (492.26,300.49) -- (510.87,309.67) -- (523.5,340.25) -- (528.5,367.75) -- (534.6,406.8) -- (461.6,400.8) ;
\draw  [draw opacity=0][dash pattern={on 0.84pt off 2.51pt}] (626.34,337.21) .. controls (617.59,348.76) and (603.71,356.23) .. (588.1,356.23) .. controls (561.63,356.23) and (540.17,334.77) .. (540.17,308.3) .. controls (540.17,286.1) and (555.27,267.42) .. (575.76,261.97) -- (588.1,308.3) -- cycle ; \draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][dash pattern={on 0.84pt off 2.51pt}] (626.34,337.21) .. controls (617.59,348.76) and (603.71,356.23) .. (588.1,356.23) .. controls (561.63,356.23) and (540.17,334.77) .. (540.17,308.3) .. controls (540.17,286.1) and (555.27,267.42) .. (575.76,261.97) ;  

\draw (580.2,286.2) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \phi $};
\draw (454.5,349.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \Phi $};
\draw (409,309) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \Phi _{\text{FP}}$};
\draw (444,288) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \tilde{\Phi }$};
\draw (516.73,264.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {$\displaystyle q+\delta $};

